LLMs as Compiler for Arabic Programming Language

In this paper we introduce APL (Arabic Programming Language) that uses Large language models (LLM) as semi-compiler to covert Arabic text code to python code then run the code. Designing a full pipeline from the structure of the APL text then a prompt (using prompt engineering) then running the prodcued python code using PyRunner. This project has a three parts first python library, a playground with simple interface and this research paper.

==> important_links.tex <==

%Riotu lab, book intro and objective 
1. https://www.riotu-lab.org/bookDetails.php?id=4

% latex and details on psronger 
2. https://www.springer.com/gp/authors-editors/book-authors-editors/manuscript-preparation/5636




